Facial Age Estimation using Convolutional Neural Networks

This paper is a part of a student project in Machine Learning at the Norwegian University of Science and Technology. In this paper, a deep convolutional neural network with five convolutional layers and three fully-connected layers is presented to estimate the ages of individuals based on images. The model is in its entirety trained from scratch, where a combination of three different datasets is used as training data. These datasets are the APPA dataset, UTK dataset, and the IMDB dataset. The images were preprocessed using a proprietary face-recognition software. Our model is evaluated on both a held-out test set, and on the Adience benchmark. On the test set, our model achieves a categorical accuracy of 52%. On the Adience benchmark, our model proves inferior compared with other leading models, with an exact accuray of 30%, and an one-off accuracy of 46%. Furthermore, a script was created, allowing users to estimate their age directly using their web camera. The script, alongside all other code, is located in our GitHub repository: AgeNet.

==> Sections/6_discussion.tex <==

\section{Future Work and Improvements} \todo{Kutte denne ned til 1/2 side? Får vi konklusjon og diskusjon inn på ish én side er vi i mål.}
\todo{Savner diskusjon av resultatene i denne seksjonen}
\label{sec:discussion}

This section suggest a different approach to the problem presented in the introduction. Furthermore, we will present two ways in which it could be relevant to explore with respect to improving our model.

\subsection{Scope of Project and Future Approaches}
From the three research papers described in Section 2, it is evident that this problem is well known and that there are numerous approaches to the problem. As a result, the method used in this paper does not have to be limiting for solving this problem and can be altered to for example an hierarchical approach or transfer learning.

Building a hierarchical model to recognise features and analyze these is something which researchers have found to be somewhat applicable \citep{pontes_et_al}. However, using a hierarchical approach will require  more mathematical insight. This is due to the use of complex mathematical processes such as the Gabor wavelets for wrinkle analysis of key facial areas. It can be argued that this approach is somewhat more mathematically challenging, than the mathematical part of our approach. For future work, a hierarchical approach will definitely be considered as a relevant scope for the method.

\iffalse
\textbf{@Christian: Avsnittet blir litt tungt å lese, :/ slik som "However, we belive that these is indeed appealing intellectual challanges inside the hierarchical method formlation.." @Erling: Gjort om og kappet nå}

\subsubsection{Transfer learning - var det dette vi drev med?}
Roth et. al. used transfer learning in order to obtain their results. Utilising a pre-trained neural network, and extracting the features the model has detected and performing analysis on these feature is a more narrow method scope than the one we used. If the approach is backed up by a well trained neural network, and is therefore solely focusing on relationships between features, it reasonable to expect a somewhat higher accuracy, compared to the accuracy attained by a our current model. Furthermore, it is understandable that some will make the argument that this approach is similar to hierarchical clustering. The difference is that the hierarchical clustering has more targeted mathematical approaches, whereas a neural network will to a greater extent be a black box. 

\textbf{@ville vært forsiktig med å si at transfer learning er et mer narrow method scope -Adrian}

\textbf{@Kan vi fjerne alt etter "Furthermore"? tror ikke vi trenger drege en paralell til den andre metoden vi snakker om. -Adrian }

\textbf{@TODO: Formuleringen i denne seksjonen gjør at det kan fremstå som mer "related work" en future work, la oss prøve å omformulere litt}
\fi


\subsection{Improving the Dataset}
A key element for training a machine learning model is the dataset on which it is trained. From section 3, it is evident that there are  shortcomings of our dataset which need addressing. From the confusion matrix, it is observable that the model often estimates both 18-22 and 23-26 as members of the 27-33 class. This can be a result of the skewedness in the data. The data is skewed to an extent where it is not representative for many populations. Therefore, it would have been highly beneficial to obtain a data which makes the key parameters aliened with the population for which we try to estimate. Secondly, more data, in terms of samples, would also improve the accuracy of the model. This is attractive and applicable as long as it doesn't further skew the distribution.

\subsection{Improving and Expanding the Methods Used}
There are numerous research papers which address features of a machine learning model which can be relevant for this problem. Some of which have not been implemented in the model presented in this paper.

A defining feature for the model are the hyperparameters. For future research, it is interesting to extend the range of the hyperparameters, in order to see if for example a deeper or wider convolutional neural network with other kernel and pooling parameters would yield improved results. In addition too review the scale of the model for a future project, one can also view new technologies for the model. One example of such can be attention. This will enable the model to strongly focus on specific parts of the data sample, and utilise knowledge about these to create a better estimation. Completed research, has shown that this can yield interesting results \citep{Wang_et_al}.

